Near-Optimal Reactive Synthesis Incorporating Runtime Information

We consider the problem of optimal reactive synthesis - compute a strategy that satisfies a mission specification in a dynamic environment, and optimizes a performance metric. We incorporate task-critical information, that is only available at runtime, into the strategy synthesis in order to improve performance. Existing approaches to utilising such time-varying information require online re-synthesis, which is not computationally feasible in real-time applications. In this paper, we pre-synthesize a set of strategies corresponding to candidate instantiations (pre-specified representative information scenarios). We then propose a novel switching mechanism to dynamically switch between the strategies at runtime while guaranteeing all safety and liveness goals are met. We also characterize bounds on the performance suboptimality. We demonstrate our approach on two examples - robotic motion planning where the likelihood of the position of the robot's goal is updated in real-time, and an air traffic management problem for urban air mobility.

==> ideas.tex <==
\section*{Story}

\begin{itemize}
    \item MDP with unknown transition probabilities. Abstract as a two-player game (probabilistic transitions abstracted as adversarial nondeterminism).
    \item We want to synthesize a strategy that satisfies a temporal logic specification in this game (surely, for all possible behaviours of the environment). 
    \item We also want the synthesized strategy to be able to make use of information provided during runtime and based on that information make decisions that are optimal with respect to the currently available knowledge about the MDP model.
    \item Introduce input variables corresponding to knowledge about parameter values (identify ranges of parameter values, then introduce input variables whose values correspond to those ranges).
    \item Associate reward values with actions/policies.
    \item Depending on parameter values, execute policy that maximizes expected reward in this case. 
\end{itemize}
\section{Problem formulation}
\begin{itemize}
    \item $\overline p$: unknown parameters in MDP $M$ with unknown transition probabilities
    \item $\mathcal F$: family of (deterministic) policies in $M$ (paremeterized by $\overline q$)
\end{itemize}

\bigskip

Goal: find a family of sets $\{R_f \subseteq Vals(\overline p)\}_{f \in \mathcal F}$ such that:
\begin{itemize}
    \item $\bigcup_{f \in \mathcal F} R_f = Vals(\overline p)$, and $R_{f_1} \neq R_{f_2}$ for all $f_1 \neq f_2$;
    \item for every $f \in \mathcal{F}$ and every $\overline r \in Vals(\overline p)$ it holds that 
    \[Reward(M_p,s,f) \geq Reward(M_p,s,f')\]
    for every $f' \in \mathcal{F}$ and $s \in S$. 
\end{itemize}

Intuitively, we would like to partition the set of possible parameter values in a way that partitions correspond to policies in $\mathcal F$, and the set of parameter valuations associated with each policy $f$ is such that $f$ is the optimal policy in the MDP corresponding to each of the parameter valuations in the set $R_f$.

\section*{Remarks}
\begin{itemize}
    \item We consider deterministic policies, as we are interested in strategies in the game abstraction of the MDP.
    \item We assume for now that policies are stationary (for the general case, we would need policies with memory).
    \item In this formulation, all policy decisions depend on all parameters in the MDP. This is normal (in known MDP the player knows the whole model), but for performance reasons it would be good to identify parameters on which individual decisions should depend.
    
\end{itemize}

\section*{Challenges}
\begin{itemize}
    \item A large number of possible policies. Not feasible to enumerate them and compute for each of them a parameter range. (Would be more efficient to associate parameter ranges with the actions in the MDP).
    \item The parameters $\overline q$ are discrete, and the parameters $\overline p$ are continuous.
\end{itemize}
\end{document}


==> old_preliminaries.tex <==
\section{Preliminaries}
\label{sec_prel}

\subsubsection{\textbf{Basic notations}}
We consider reactive systems with a finite set
$\inp$ ($\out$) of Boolean \emph{inputs (outputs)}.
The input alphabet is
$\ialphabet=2^\inp$, the output alphabet is $\oalphabet=2^O$, and
$\alphabet=\ialphabet \times \oalphabet$. The set of finite (infinite) words
over $\alphabet$ is denoted by $\alphabet^*$ ($\alphabet^\omega$), and
we define $\alphabet^{\infty} = \alphabet^* \cup \alphabet^\omega$.  We will also refer
to words as \emph{(execution) traces}\todo{Can we stick to
one?}.  We write $|\trace|$ for the
length of a trace $\trace\in \alphabet^*$. For an infinite trace $\trace\in \alphabet^\omega$ we define $|\trace| =\infty$. For $\itrace = x_0
x_1 \ldots \in \ialphabet^\infty$ and $\otrace = y_0 y_1 \ldots \in
\oalphabet^\infty$, we write $\itrace \parallel \otrace$ for the
composition $(x_0,y_0) (x_1,y_1) \ldots \in \alphabet^\infty$.
For $i \in \nats$ and a word $\trace = \sigma_0\sigma_1\ldots \in \awords\Sigma$, we define $\trace[i] = \sigma_i$, and we define $\trace[i,j) = \sigma_i\sigma_{i+1}\ldots\sigma_{j-1}$ if $j \in \nats$ and $\trace[i,j) = \sigma_i\sigma_{i+1}\ldots$ if $j = \infty$.
A \emph{language} is a set $\lang
\subseteq  \alphabet^\infty$ of words.
\todo{Are we using all the notations?}
%We denote the set of all languages as $\langset = 2^{\alphabet^\infty}$.

\iffalse
\subsubsection{Reactive systems}

A \emph{reactive system} is defined by a
6-tuple $\proc = (\states,q_{0},\ialphabet,\oalphabet,\delta,\lambda)$,
where
$\states$ is a finite set of states,
$q_{0} \in \states$ is the initial state,
$\ialphabet$ is the input alphabet,
$\oalphabet$ is the output alphabet,
$\delta: \states \times \Sigma_{\inp} \to \states$ is the complete transition function, and $\lambda : \states \times \Sigma_{\inp} \to \Sigma_{\out}$ is the output function.
%
Given an input trace $\itrace = x_0 x_1 \ldots \in \ialphabet^\infty$, a reactive system $\mathcal{\proc}$ produces an
output trace $\otrace = \mathcal{\proc}(\itrace) = \lambda(q_0, x_0)
\lambda(q_1, x_1) \ldots \in \oalphabet^\infty$ with $q_{i+1} = \delta(q_i, x_i)$ for all $i \ge 0$.
The set of words produced by
$\mathcal{\proc}$ is denoted $\lang(\mathcal{\proc}) = \{\itrace \parallel \otrace \in
\alphabet^\infty \mid \mathcal{\proc}(\itrace) = \otrace\}$.


\subsubsection{Serial composition of reactive systems}
Consider two reactive systems  $\proc = (\states,q_{0},\ialphabet,\oalphabet,\delta,\lambda)$ and $\shield = (\states', q_{0}',\ialphabet\times\oalphabet, \oalphabet,\delta',\lambda')$.
The \emph{serial composition} of $\proc$ and $\shield$ is obtained by feeding the input and output of $\proc$ to $\shield$ and results in a new reactive system $\proc \comp \shield=(\hat{\states}, \hat{q_{0}}, \ialphabet,\oalphabet, \hat{\delta},
\hat{\lambda})$, where
   $\hat{\states} = \states \times \states'$,
   $\hat{q_{0}} = (q_{0}, q_{0}')$,
   $\hat{\delta}((q,q'),\isymb) = (\delta(q,\isymb), \delta'(q',(\isymb,\lambda(q,\isymb))))$, and
   $\hat{\lambda}((q,q'),\isymb) = \lambda'(q',(\isymb,\lambda(q, \isymb)))$.

   
\subsubsection{Multi-agent reactive systems}
A \emph{multi-agent reactive system} $\proc$ is a tuple $(\proc, \ialphabet,  \oalphabet)$, where $\proc = \{\proc_1,\ldots,\proc_n\}$ is a set of agents, where each $\proc_i = (\states_i, q_{0,i},\ialphabeti,\oalphabeti,\delta_i,\lambda_i)$ is a reactive system.
%
While multiple agents may be able to read the same input variables to indicate
broadcast from the environment, the sets of outputs are pairwise disjoint: for $i \neq j$, we have $\out_i \cap \out_j = \emptyset$. Furthermore, agents cannot directly read each others outputs, that is, for all $i$ and $j$, we have $\out_i \cap \inp_j = \emptyset$. The outputs of the multiagent system  $\proc$ are $\out = \bigcup_{i=1}^n \out_i$, and its inputs are $\inp  = \bigcup_{i=1}^n \inp_i$.
%
The joint behaviour of the multi-agent system is a reactive system 
$\proc=(\states, q_{0}, \ialphabet,\oalphabet, \delta,
\lambda)$ defined as follows: the set $\states = \bigotimes_i \states_i$ of states is formed by the product of
the states of all agents $\proc_i \in \proc$. The initial state $q_{0}$ is formed
by the initial states $q_{0,i}$ of all $\proc_i \in \proc$. The transition function $\delta$ updates, for each agent $\proc_i \in \proc$, the $\states_i$ part of the state in accordance with the transition function $\delta_i$, using
the projection $\symb(I_i)$ as input. The output function $\lambda$ labels each state with the
union of the outputs of all $\proc_i \in \proc$ according to $\lambda_i$.



\subsubsection{Specifications}

A \emph{specification} $\spec$ defines a set $\lang(\spec) \subseteq \alphabet^\infty$ of allowed traces.
%
A reactive system $\proc$ \emph{realizes} $\spec$, denoted by $\proc \models \spec$, iff
$\lang(\proc) \subseteq \lang(\spec)$.
Given a set of propositions $\mathsf{AP}$, a formula in \emph{linear temporal logic} (LTL) describes a language in $(2^\mathsf{AP})^\omega$. LTL extends Boolean logic by the introduction of temporal operators such as $\LTLnext$ (next time), $\LTLglobally$ (globally), $\LTLfinally$ (eventually), and $\LTLuntil$ (until)~\cite{Pnueli77}.
%
$\varphi$ is called a \emph{safety specification} if every trace $\trace$ that is not in  $\lang(\spec)$  has a prefix $\tau$ such that all words starting with $\tau$ are also not in the language $\lang(\spec)$.
We represent a safety specification $\varphi$ by a safety automaton
$\varphi = (Q, q_0, \alphabet, \delta, F)$, where $F\subseteq Q$ is a set of safe states.
\fi

\subsubsection{\textbf{Linear temporal logic}}
A linear temporal logic formula $\spec$ defines a set $\lang(\spec) \subseteq \alphabet^\infty$ of allowed traces. $\varphi$  is generated by the grammar\\
\[\varphi := p \mid \true \mid \false \mid \varphi \wedge \varphi \mid \varphi \vee \varphi \mid \LTLnext  \varphi  \mid \varphi \LTLuntil \varphi \mid \varphi \LTLrelease \varphi,\]\\
where $p \in \Sigma$ is an atomic proposition, $\LTLnext$ is the \emph{next} operator, $\LTLuntil$ is the \emph{until} operator, and $\LTLrelease$ is the \emph{release} operator. We also define the derived operators 
\emph{finally}, defined as $\LTLfinally \varphi = \true \LTLuntil \varphi$ and 
\emph{globally}, defined as $\LTLglobally \varphi = \false \LTLrelease \varphi$.
LTL formulas are interpreted over (infinite) runs. If a trace $\pi$ satisfies an LTL formula $\varphi$, we write $\pi \models \varphi$. The formal definition of LTL semantics can be found in~\cite{BaierKatoen08}.

\subsubsection{\textbf{Games}}
%
The game is played by two players --- the agent and the
environment. It is characterized by the tuple $\game = (\gstates,
\ginit, \ialphabet, \oalphabet, \delta,\mathcal L, \Acc)$,
where $\gstates$ is a finite set of states, $\ginit \in
\gstates$ is the initial state, $\ialphabet, \oalphabet$ are
the alphabets available to the environment and the agent respectively, 
$\delta: \gstates \times \alphabet \rightarrow \gstates$
is a complete transition function, $\mathcal L:\gstates
\rightarrow \ialphabet \times \oalphabet$ is the labeling
function, and $\Acc: \playDomain \rightarrow \bools$ is a
winning condition. 
%and defines the qualitative objective of
%the game, and $\Val: \playDomain \rightarrow \mathbb{R}$ is
%a value function defining the quantitative objective of the
%game. 
%\todo[inline]{Should we replace qualitiative with
%feasibility and quantitative with objective?}
%A game can have a
%winning condition, a value function, or
%both.\todo[inline]{Is this optionality really important? Can't we
%set $\Acc$ to be always true or $\Val$ function to be always
%zero?}
%

The game is played  by two players: the agent and the
environment. In every state $g\in \gstates$ (starting with
$\ginit$), the environment chooses an input $\isymb \in
\ialphabet$, and then the agent chooses some output $\osymb
\in \oalphabet$. These choices define the next state $g' =
\delta(g,(\isymb, \osymb))$, and so on. The resulting
(infinite) sequence $\overline{\pi} = (g_0,\isymb, \osymb,
g_1) (g_1,\isymb, \osymb, g_2) \ldots$ is called a
\emph{play}\todo{Should we mention why does agent get the
    second chance?  Because of reactivity?}.  A
    deterministic  \emph{strategy} for the environment is a
    function $\rho_e: \gstates^* \rightarrow \ialphabet$.  A
    nondeterministic (deterministic) \emph{strategy} for the
    agent is a relation $\rho_s: \gstates^* \times
    \ialphabet \rightarrow 2^{\oalphabet}$  (function
    $\rho_s: \gstates^* \times \ialphabet \rightarrow
    \oalphabet$).\todo{What is $\gstates^*$?} A strategy is
    \emph{winning} for the agent if all plays
    $\overline{\pi}$ that can be constructed when defining
    the outputs using the strategy result in
    $\Acc(\overline{\pi})=\top$. 

%\todo[inline]{Is the remainder of this section equivalent to
%the following max-min optimization problem? Here, $\Pi:
%\mathcal{P}_s\times \mathcal{P}_e \rightarrow \playDomain$
%Will we be using the terminology introduced?}
%\begin{subequations}
%    \begin{align}
%        \underset{\rho_e}{\mathrm{max}}\ \underset{\rho_s}{\mathrm{min}}&\quad
%        \Val(\Pi(\rho_s,\rho_e) )\\
%        \mathrm{subject\ to}&\quad \rho_s\in\mathcal{P}_s\\
%   						    &\quad \rho_e\in\mathcal{P}_e\\
%                            &\quad
%                            \Pi(\rho_s,\rho_e)\models \varphi
%    \end{align}%
%\end{subequations}%
%
%A play $\overline{\pi}$ is \emph{won} by the system iff $\Acc(\overline{\pi})=\top$. We assume our acceptance conditions are given as LTL formulas. Hence, for a game $\game$ and LTL formula $\spec$ we will have $\Acc(\overline{\pi})=\top$ iff $\overline{\pi} \models \varphi$.
%
%
% A strategy is \emph{winning} for the system if all plays $\overline{\pi}$ that can be
%constructed when defining the outputs using the strategy result in
%$\Acc(\overline{\pi})=\top$. The \emph{winning region} $\Win$ is the set of states
%from which a winning strategy exists.
%

% A \emph{safety game} defines $\Acc$ via a set $F\subseteq \gstates$ of
% safe states: $\Acc(\overline{\pi})=\top$ iff $g_i \in F$ for all $i \geq 0$, i.e., if only safe states are visited in the play $\overline{\pi}$. Otherwise, $\Acc(\overline{\pi})=\bot$.
% %If a safety game is won by the system player, then there exists a permissive strategy $\rho_s$ that is \emph{memoryless}, i.e., has the form $\rho_s:
% %\gstates \times \ialphabet \rightarrow 2^{\oalphabet}$.
% %
% The \emph{\buchi} winning condition is $\Acc(\overline{\pi})=\top$ iff $\inf(\overline{\pi})
% \cap F \neq \emptyset$, where $F \subseteq G$ is
% the set of accepting states and $\inf(\overline{\pi})$ is the set of states that occur infinitely often in $\overline{\pi}$.
% We abbreviate the \buchi condition as $\mathcal{B}(F)$.
% A \emph{Generalized Reactivity 1} (GR(1))
% acceptance condition is a predicate $\bigwedge_{i=1}^{m} \mathcal{B}(E_{i}) \rightarrow \bigwedge_{i=1}^{n} \mathcal{B}(F_{i})$, with
% $E_i \subseteq G$ and $F_i \subseteq G$.

%The quantitative objective of the system is to minimize $\Val(\overline{\pi})$.\looseness=-1

% %
% \iffalse MEAN-PAYOFF
% A \emph{mean-payoff game} is a game where $\Val$ is defined via an edge labeling function $r :
% \delta \rightarrow \{-W,\dots, W\}$, which assigns values between $-W$ and $W$ to edges. For a play $\pi =
% e_0 e_1 e_2 \dots \in \delta^\omega, \Val(\overline{\pi}) = \lim \sup_{n\rightarrow\infty} \frac{1}{n+1} \sum_{i=0}^{n} r(e_i)$.
% \fi
% 
% 
% 



==> old_prob_st.tex <==
\begin{definition}[Optimizing proposition]
Similar to \cite{smith2011optimal} we first define an \emph{optimizing proposition} $p \in \Sigma$. Given a game $\mathcal G$, we consider LTL formulas of the form

\begin{equation}
\label{eq:temp_spec}
\spec:=\bigwedge_{i=1}^{m} \mathcal{B}(E_{i}) \rightarrow \left(\phi \wedge \LTLglobally\,\LTLfinally\, p\right).
\end{equation}
with $E_i \subseteq G$

\end{definition}

Adding cost information does not change the ability of a system to satisfy a specification. Since there is, in general, no unique satisfying strategy, cost information typically conveys a \emph{preference} over correct strategies. We formally define this notion in the following. 
\begin{definition}[Preference vector]
Given a game $\game$, with $\Acc$ given by LTL formula $\varphi$, we denote finite set of strategies $\rho \in \mathcal{R}$ such that the corresponding induced set of plays $\Pi \subseteq \mathcal{L}(\game)$  $\pi \models \varphi$ for all $\pi \in \Pi$. We define the corresponding \emph{cost vector} $\mathbf{C}:\Pi \rightarrow \mathbb{R}^N$ associated with the set of policies as $C = \{\Val(\pi_i),\ldots,\Val(\pi_n)\}$. 

We now define a preference vector $\mathbf{p} \in \mathbb{R}^n$ to be a weighting over the corresponding policies in $\Pi$

 
\end{definition}

The preference vector can lie in the continuous space. For example, the preference vector can be probabilities associated with knowledge being gained during runtime. 

Intuitively, this vector can be used to direct the agent to behave more optimally as information is provided. Informally, we are interested in using this vector to choose the strategy in the set $\Pi$ that is the \emph{most optimal} given the current value of $p$. 

We make the notion of optimality more concrete in the following

\begin{definition}[Weighted value function]
Given a particular $\overline{p} \in \mathbb{R}^n$
\end{definition}

Consider a winning play $\pi_i \in \Pi$ for LTL formula given in Equation \ref{eq:temp_spec}. 
We are interested in all time instances when proposition $p$ is satisfied. 


Let $\pi_p[i]$ be the $ith$ instance when $p = \top$. For some $j > i$, we define cost function 
\begin{equation}
    C(\pi_p[i,j]) = \sum_{k=i}^{j-1}\pi[k]
\end{equation}
Simply, $C$ is a cost function defined over intervals of satisfying the optimizing proposition. 

We define the quantitative objective of the system as the following
\begin{equation}
    C(\pi_p[i,j]) = \sum_{k=i}^{j-1}\pi[k]
\end{equation}


\begin{prob}
    Given a game $ \mathcal{G}$, strategies for the system $ \overline{\rho_s}_i$
    synthesized for weights $ \overline{q}_i\in
    \mathcal{S}_L$ for $i\in\{1,2,\ldots,N\}$, and a query
    weight $\overline{p}\in \mathcal{S}_L$, identify the
    policy $\pi_i$ such that for some user-specified
    $\epsilon >0$,
    \begin{align}
        V^{\pi_i}(s_0; \overline{p})\leq
        \max_{\pi\in\Pi}
        V^{\pi}(s_0; \overline{p}) \leq V^{\pi_i}(s_0;
        \overline{p}) + \epsilon,\ \forall s_0\in \mathcal{S}
    \end{align}
    Here, $\Pi$ denotes all the admissible policies that
    satisfy some pre-determined specifications.
\end{prob}



==> synthesis.tex <==
% In this section, we present a method to synthesize candidate policies that are optimal for specific instantiations of the runtime information vector. In the next section, we show how we switch between the policies at runtime to obtain more optimal behaviour. 


% We follow the convention of \cite{hadaspaper,rudigerpaper}. \todo[inline]{elaborate from Kress-grazit robotics papers.}
